LDQL: A Query Language for the Web of Linked Data (Extended Version)

The Web of Linked Data is composed of tons of RDF documents interlinked to each other forming a huge repository of distributed semantic data. Effectively querying this distributed data source is an important open problem in the Semantic Web area. In this paper, we propose LDQL, a declarative language to query Linked Data on the Web. One of the novelties of LDQL is that it expresses separately (i) patterns that describe the expected query result, and (ii) Web navigation paths that select the data sources to be used for computing the result. We present a formal syntax and semantics, prove equivalence rules, and study the expressiveness of the language. In particular, we show that LDQL is strictly more expressive than the query formalisms that have been proposed previously for Linked Data on the Web. The high expressiveness allows LDQL to define queries for which a complete execution is not computationally feasible over the Web. We formally study this issue and provide a syntactic sufficient condition to avoid this problem; queries satisfying this condition are ensured to have a procedure to be effectively evaluated over the Web of Linked Data.

==> ldql-proposal.tex <==
\section*{Proposal}
\label{sec:Proposal}



\subsection*{(NEW) LDQL Queries and Link Path Expressions}

$\symPattern$ is a SPARQL graph pattern, $U$ is a set of URIs, $?x,?v$ are variables,
and $\symLP$ is a link pattern.
The syntax of LDQL queries is given by the following rules.

\begin{align*}
	\symQuery \, \definedAs \, \, & \tuple{\symLPE,\symPattern} 
	\,\mid\, (\symQuery \OpAND \symQuery )
	\,\mid\, (\symQuery \OpUNION \symQuery )
	\,\mid\, (\OpSEED\ U\ \symQuery )
	\,\mid\, (\OpSEED\ ?v\ \symQuery ) \\
	\symLPE \, \definedAs \, \, &
		\peEmpty
	\,\mid\,
		\symLP
	\,\mid\,
		(?x, \symQuery)
	\,\mid\,
		\peConcat{\symLPE}{\symLPE}
	\,\mid\,
		\peAlt{\symLPE}{\symLPE}
	\,\mid\,
		\peKleene{\symLPE}
	\,\mid\,
		%\peTest{\symQuery}
		\peTest{\symLPE}
\end{align*}%

For the semantics, besides a Web of Linked Data $W$, every query is given a set $S$ of seed URIs 
(from ``outside'' the query). 
Thus for a query $\symQuery$ we define $\fctEvalQW{  \symQuery  }{\symWoD}^S$
as follows.
\begin{align*}
	\fctEvalQW{\tuple{\symLPE,\symPattern}}{\symWoD}^S & \definedAs
	\fctEvalPGD{\symPattern}{}{\symRDFdataset}	
	\;\;\; \text{ where }\symRDFdataset=\dataset\big( \textstyle \bigcup_{u\in S}\fctEvalPathPdW{\symLPE}{u}{\symWoD}\big)
  \\
	\fctEvalQW{(\OpSEED\ U\ \symQuery )}{\symWoD}^S & \definedAs
	\fctEvalQW{\symQuery }{\symWoD}^U
	\\
	\fctEvalQW{(\OpSEED\ ?v\ \symQuery )}{\symWoD}^S & \definedAs
		\textstyle \bigcup_{\symURI \in \symAllURIs} \bigl( \fctEvalQW{\symQuery}{\symWoD}^{\lbrace \symURI \rbrace} 
		\Join \lbrace ?v\to \symURI \rbrace \bigr)
\end{align*}
The semantics for $\OpAND$ and $\OpUNION$ is defined as usual.
In the above definition the operator $\dataset(\cdot)$ takes a set $U$ of URIs as input, 
and produces an RDF dataset with named graphs $(u,\fctData{u})$%
\footnote{I'm using $\fctData{u}$ as a shorthand for $\fctData{\fctADoc{u}}$}
for every $u\in U\cap \fctDom{\fctsymADoc}$, and default graph 
constructed as the merge of all $\fctData{u}$ for all $u\in U\cap \fctDom{\fctsymADoc}$.
To complete the definition of the semantics of LDQL we only need to define the
semantics of a Link Path Expressions which is given by the following rules.
\begin{align*}
	\fctEvalPathPdW{\,\peEmpty\,}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symCtxURI \rbrace
	\\
	\fctEvalPathPdW{p}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symURI \,|\, \text{exists }(\symCtxURI,p,\symURI) \in \fctData{\symCtxURI} \rbrace	
	\\
	\fctEvalPathPdW{\symLP}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symURI \,|\, \text{exists }\tuple{\symCtxDoc,t,\symURI,d} \in \G(\symWoD) \text{ that matches $\symLP$ in the context of } \symCtxURI \rbrace
	\\[-0.7mm] % Layout Adjustment
	\fctEvalPathPdW{\peConcat{\symLPE_1}{\symLPE_2}}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symURI \in \fctEvalPathPdW{\symLPE_2}{\symURI'}{\symWoD} \,|\, \symURI' \in \fctEvalPathPdW{\symLPE_1}{\symCtxURI}{\symWoD} \rbrace
	\\
	\fctEvalPathPdW{\peAlt{\symLPE_1}{\symLPE_2}}{\symCtxURI}{\symWoD} &\definedAs
		\fctEvalPathPdW{\symLPE_1}{\symCtxURI}{\symWoD} \cup \fctEvalPathPdW{\symLPE_2}{\symCtxURI}{\symWoD}
	\\
	\fctEvalPathPdW{\peKleene{\symLPE}}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symCtxURI \rbrace \cup \fctEvalPathPdW{\symLPE}{\symCtxURI}{\symWoD} \cup \fctEvalPathPdW{\peConcat{\symLPE}{\symLPE}}{\symCtxURI}{\symWoD} \cup \fctEvalPathPdW{\peConcat{\peConcat{\symLPE}{\symLPE}}{\symLPE}}{\symCtxURI}{\symWoD} \cup \ldots
	\\
		\fctEvalPathPdW{\,(?x,\symQuery)\,}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symURI\in \symAllURIs \mid \text{ there exists }\mu\in\fctEvalQW{\symQuery}{\symWoD}^{{\lbrace \symCtxURI \rbrace}} 
		\text{ such that }\mu(?x)=\symURI  \rbrace 
\\
	\fctEvalPathPdW{\,\peTest{\symLPE}\,}{\symCtxURI}{\symWoD} &\definedAs
		\lbrace \symURI \,|\, \fctEvalPathPdW{\symLPE}{ \symURI }{\symWoD} \neq \emptyset \text{ and }\symURI=\symCtxURI\rbrace
	.
\end{align*}


